Detectability of Supernova Remnants with the Southern Wide-field Gamma-ray Observatory

Supernova remnants (SNRs) are likely sources of hadronic particle acceleration within our galaxy, contributing to the galactic cosmic ray flux. Next-generation instruments, such as the Southern Wide-field Gamma-ray Observatory (SWGO), will be of crucial importance in identifying new candidate SNRs. SWGO will observe two-thirds of the gamma-ray sky, covering the energy range between a few hundreds of GeV and a PeV. In this work, we apply a model of SNR evolution to a catalogue of SNRs in order to predict their gamma-ray spectra, explore the SNR emission phase space, and quantify detection prospects for SWGO. Finally, we validate our model for sources observed with current-generation instruments, fitting it using a Monte-Carlo Markov Chain technique to the observed gamma-ray emission from four SNRs. We anticipate that at least 6, and potentially as many as 11 SNRs will be detected by SWGO within 1 year.

==> jcap_example.tex <==
\section{Some examples}
\label{sec:intro}

For internal references use label-refs: see section~\ref{sec:intro}.
Bibliographic citations can be done with "cite": refs.~\cite{a,b,c}.
When possible, align equations on the equal sign. The package
\texttt{amsmath} is already loaded. See \eqref{eq:x}.
\begin{equation}
\label{eq:x}
\begin{aligned}
x &= 1 \,,
\qquad
y = 2 \,,
\\
z &= 3 \,.
\end{aligned}
\end{equation}
Also, watch out for the punctuation at the end of the equations.


If you want some equations without the tag (number), please use the available
starred-environments. For example:
\begin{equation*}
x = 1
\end{equation*}

\section{Figures and tables}

All figures and tables should be referenced in the text and should be
placed on the page where they are first cited or in
subsequent pages. Positioning them in the source file
after the paragraph where you first reference them usually yield good
results. See figure~\ref{fig:i} and table~\ref{tab:i} for layout examples. 
Please note that a caption is mandatory  and it must be placed at the bottom of both figures and tables.

\begin{figure}[htbp]
\centering
\includegraphics[width=.4\textwidth]{example-image-a}
\qquad
\includegraphics[width=.4\textwidth]{example-image-b}
\caption{Always give a caption.\label{fig:i}}
\end{figure}

\begin{table}[htbp]
\centering
\begin{tabular}{lr|c}
\hline
x&y&x and y\\
\hline
a & b & a and b\\
1 & 2 & 1 and 2\\
$\alpha$ & $\beta$ & $\alpha$ and $\beta$\\
\hline
\end{tabular}
\caption{We prefer to have top and bottom borders around the tables.\label{tab:i}}
\end{table}

We discourage the use of inline figures (e.g. \texttt{wrapfigure}), as they may be
difficult to position if the page layout changes.

We suggest not to abbreviate: ``section'', ``appendix'', ``figure''
and ``table'', but ``eq.'' and ``ref.'' are welcome. Also, please do
not use \texttt{\textbackslash emph} or \texttt{\textbackslash it} for
latin abbreviaitons: i.e., et al., e.g., vs., etc.


\paragraph{Up to paragraphs.} We find that having more levels usually
reduces the clarity of the article. Also, we strongly discourage the
use of non-numbered sections (e.g.~\texttt{\textbackslash
  subsubsection*}).  Please also consider the use of
``\texttt{\textbackslash texorpdfstring\{\}\{\}}'' to avoid warnings
from the \texttt{hyperref} package when you have math in the section titles.

%% or
%% [B] Manual formatting (see below)
%% (i) We suggest to always provide author, title and journal data or doi:
%% in short all the informations that clearly identify a document.
%% (ii) please avoid comments such as "For a review'', "For some examples",
%% "and references therein" or move them in the text. In general, please leave only references in the bibliography and move all
%% accessory text in footnotes.
%% (iii) Also, please have only one work for each \bibitem.

\begin{thebibliography}{99}

\bibitem{a}
Author,
\emph{Title},
\emph{J. Abbrev.} {\bf vol} (year) pg.

\bibitem{b}
Author,
\emph{Title},
arxiv:1234.5678.

\bibitem{c}
Author,
\emph{Title},
Publisher (year).

\end{thebibliography}

==> table_SNRs.tex <==
%\begin{adjustbox}{angle=90}
\begin{table*}
\begin{tabular}{clccccccc}
% Source &
%   \multicolumn{1}{c}{Name} &
%   \begin{tabular}[c]{@{}c@{}}Detectable\\ after 1\,yr\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Detectable\\ after 5\,yr\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Detectable\\ by HESS\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Detected\\ by HESS\end{tabular} &
%   Location &
%   \begin{tabular}[c]{@{}c@{}}Flux\\ for $E$ > 1 TeV\\ (TeV cm$^-2$ s$^-1$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Flux\\ for $E$ > 10 TeV\\ (TeV cm$^-2$ s$^-1$)\end{tabular} \\ 

Source &
  \multicolumn{1}{c}{Name} &
  \begin{tabular}[c]{@{}c@{}}SWGO\\ 1\,yr\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}SWGO\\ 5\,yr\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}HESS\\ 50 hrs \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Detected\\ by HESS\end{tabular} &
  Loc. &
  \begin{tabular}[c]{@{}c@{}}Flux\\ $E>1$ TeV\\ (TeV cm$^-2$ s$^-1$) \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Flux\\ $E>10$ TeV\\ (TeV cm$^-2$ s$^-1$) \end{tabular} \\ 
\hline
G347.3-00.5 & RX J1713.7-3946                  & Yes & Yes & Yes & Yes   & SH & 1.67e-10 & 5.39e-11 \\
G327.6+14.6 & SN1006              & Yes & Yes & Yes & Yes   & SH & 6e-11    & 2.54e-11 \\
G266.2-01.2 & Vela Jr         & Yes & Yes & Yes & Yes   & SH & 1.04e-10 & 1.17e-11 \\
G120.1+01.4 & Tycho              & Yes & Yes & Yes & No    & NH & 4.51e-12 & 3.44e-12 \\
G260.4-03.4 & Puppis A              & Yes & Yes & Yes & (Yes) & SH & 2.05e-11 & 1.6e-12  \\
G309.2-00.6 &                                  & Yes & Yes & Yes & No    & SH & 2.19e-12 & 8.89e-13 \\
G315.4-02.3 & RCW 86                & Yes & Yes & Yes & Yes   & SH & 2.73e-12 & 6.95e-14 \\
G089.0+04.7 & HB21                             & Yes & Yes & Yes & No    & NH & 2.01e-12 & 8.49e-16 \\
G111.7-02.1 & Cas. A             & No  & Yes & No  & No    & NH & 1.16e-12 & 9.51e-13 \\
G015.9+00.2 &                                  & No  & Yes & Yes & No    & SH & 7.59e-13 & 2.3e-13  \\
G332.5-05.6 &                                  & No  & Yes & Yes & No    & SH & 1.2e-12  & 5.07e-14 \\
G038.7-01.3 &                                  & No  & Yes & Yes & No    & NH & 6.93e-13 & 4.21e-14 \\
G166.0+04.3 & VRO 42.05.01                     & No  & Yes & Yes & No    & NH & 5.86e-13 & 5.96e-15 \\ 
\hdashline
G027.4+00.0 & (Kes 73), 4C-04.71               & No  & No  & No  & (Yes) & SH & 1.68e-13 & 1.2e-13  \\
G033.6+00.1 & Kes 79            & No  & No  & No  & No    & NH & 1.98e-13 & 9.27e-14 \\
G109.1-01.0 & CTB 109                          & No  & No  & Yes & No    & NH & 6.11e-13 & 7.06e-14 \\
G322.1+00.0 & Circinus X-1                     & No  & No  & No  & No    & SH & 1.51e-13 & 6.61e-14 \\
G272.2-03.2 &                                  & No  & No  & Yes & No    & SH & 4.27e-13 & 4.83e-14 \\
G352.7-00.1 &                                  & No  & No  & No  & No    & SH & 9.73e-14 & 4.7e-14  \\
G032.8-00.1 & Kes 78                           & No  & No  & No  & (Yes)   & SH & 1.51e-13 & 2.63e-14 \\
G084.2-00.8 &                                  & No  & No  & No  & No    & NH & 3.07e-13 & 2e-14    \\
G346.6-00.2 &                                  & No  & No  & No  & No    & SH & 5.3e-14  & 1.71e-14 \\
G116.5+01.1 &                                  & No  & No  & Yes & No    & NH & 3.68e-13 & 1.01e-14 \\
G021.8-00.6 & Kes 69                           & No  & No  & Yes & No    & SH & 3.91e-13 & 9.37e-15 \\
G337.8-00.1 & Kes 41                           & No  & No  & No  & No    & SH & 6.89e-14 & 7.88e-15 \\
G028.6-00.1 &                                  & No  & No  & No  & (Yes)   & SH & 5.8e-14  & 6.09e-15 \\
G327.4+00.4 & Kes 27                           & No  & No  & No  & No    & SH & 2.1e-13  & 4.45e-15 \\
G355.6-00.0 &                                  & No  & No  & No  & No    & SH & 2.59e-14 & 2.97e-15 \\
G094.0+01.0 & 3C434.1                          & No  & No  & No  & No    & NH & 9.46e-14 & 2.54e-15 \\
G296.7-00.9 &                                  & No  & No  & No  & No    & SH & 1.08e-13 & 1.22e-15 \\
G085.9-00.6 &                                  & No  & No  & No  & No    & NH & 5.55e-14 & 9.98e-16 \\
G296.1-00.5 &                                  & No  & No  & Yes & No    & SH & 1.91e-13 & 7.89e-16 \\
G284.3-01.8 & MSH 10-53                        & No  & No  & Yes & Yes   & SH & 2.61e-13 & 7.41e-16 \\
G046.8-00.3 & (HC30)                           & No  & No  & No  & No    & NH & 1.16e-13 & 5.25e-16 \\
G053.6-02.2 & 3C400.2, NRAO 611                & No  & No  & No  & No    & NH & 3.37e-14 & 6.44e-17 \\
G357.7+00.3 & the Square                       & No  & No  & Yes & No    & SH & 9.63e-14 & 8.53e-18 \\
G359.1-00.5 &                                  & No  & No  & No  & (Yes)   & SH & 1.63e-14 & 2.36e-19 \\
G082.2+05.3 & W63                              & No  & No  & Yes & No    & NH & 7.46e-14 & 2.79e-20
\end{tabular}
\caption{All 38 SNRs sorted by their detectability according to figure \ref{fig:sedstypvals}}
\label{tab:SNRlist}
\end{table*}
%\end{adjustbox}
